Photoemission Beyond the Sudden Approximation

The many-body theory of photoemission in solids is reviewed with emphasis on methods based on response theory. The classification of diagrams into loss and no-loss diagrams is discussed and related to Keldysh path-ordering book-keeping. Some new results on energy losses in valence-electron photoemission from free-electron-like metal surfaces are presented. A way to group diagrams is presented in which spectral intensities acquire a Golden-Rule-like form which guarantees positiveness. This way of regrouping should be useful also in other problems involving spectral intensities, such as the problem of improving the one-electron spectral function away from the quasiparticle peak.

==> pics/Makefile <==
# Makefile for .eps files
# $Id: Makefile,v 1.2 2005/10/31 14:59:51 coa Exp $

EPSFILES = pe0.eps pe1.eps noloss.eps p_gen.eps contour.eps m1.eps \
   m2.eps m1b.eps

all: $(EPSFILES)

.SUFFIXES: .eps .tex

.tex.eps:
	feynmf $*
	xdvi $*
	dvips -E -o $@ $*.dvi

print: all
	@for i in $(EPSFILES); do\
	    echo $(LP) $$i; \
	    $(LP) $$i; \
	done

clean:
	rm -f *.aux *.log *.dvi *.*gf *.mf *.tfm *.*pk *.shar ?.*

spotless: clean
	rm -f *.eps

dist:
	shar *.tex Makefile > fig.shar 


